Group pattern detection of longitudinal data using functional statistics

Estimations and evaluations of the main patterns of time series data in groups benefit large amounts of applications in various fields. Different from the classical auto-correlation time series analysis and the modern neural networks techniques, in this paper we propose a combination of functional analysis of variance (FANOVA) and permutation tests in a more intuitive manner for a limited sample size. First, FANOVA is applied in order to separate the common information and to dig out the additional categorical influence through paired group comparison, the results of which are secondly analyzed through permutation tests to identify the time zones where the means of the different groups differ significantly. Normalized kernel functions of different groups are able to reflect remarkable mean characteristics in grouped unities, also meaningful for deeper interpretation and group-wise classification. In order to learn whether and when the proposed method of FANOVA and permutation F-test works precisely and efficiently, we compare the estimated kernel results with the ground truth on simulated data. After the confirmation of the model's efficiency from simulation, we apply it also to the RAVDESS facial dataset to extract the emotional behaviors of humans based on facial muscles contractions (so-called action units (AU) technically in computer graphics), by comparing the neutral performances with emotional ones.

==> 1_introduction.tex <==



The study of human facial expressions and emotions never stops in our daily life while we communicate with others. Following the increased interest in automatic facial behavior analysis and understanding, the need of a semantic interpretation of the evolution of facial expressions and of human emotions has become of interest in recent years \cite{Fridlun2014}. In this paper, based on a work cooperated with the Serbian company 3Lateral, which has special expertise on building visual styles and designs in animation movies, we want to explore functional statistical instruments to identify the emotions while analyzing the expressions through recorded videos of human faces. The final aim of this research is to use this information to better and more realistically establish virtual digital characters, able to interact autonomously with real humans. 

The data that we consider are multivariate longitudinal data, showing the evolution in time of different face muscles contraction. Functional Data Analysis (FDA) offers the possibility to analyze the entire expression evolution process over time and to gain detailed and in-depth insight into the analysis of emotion patterns. The basic idea in functional data analysis is that the measured data are noisy observations coming from a smooth function. Ramsay and Silverman \cite{ramsay1997functional} describe the main features of FDA, that can be used to perform exploratory, confirmatory or predictive data analysis. Ullah and Finch \cite{UllahShahid2013} published a systematic review on the applications of functional data analysis, where they included all areas where FDA was applied.

%Since the videos unavoidably have different beginning and ending points, the observed values are not comparable vertically among videos. Patterns of the expression functions common to each emotion are obscured due to the misalignment in the original data but can be clearer after curves are aligned\cite{marron2015functional}. It is essential to align the unregistered chronological timeline in the dataset into a common registered internal timeline that follows the same pronunciation speed, to control the influence of the speech itself, and then to study the influence of the emotions.


In our application, functional analysis of variance (FANOVA) can be used to determine if there are time-related differences between emotion groups by using a functional F-test \cite{Dannenmaier2020}. %FANOVA yields the possibility to determine if a functional response can be described by scalar or functional variables.

%The structure of this paper goes as follows. In this chapter, in Section 2 we briefly describe the pre-processing steps. Section 3 includes the knowledge of functional univariate multiple linear regression and FANOVA, and permutation F-test is introduced in Section 4. Chapter 2 illustrates the simulation process and results, while in chapter 3 we apply the method on RAVDESS dataset from where the expression data of interest is extracted and studied.



%\textbf{old part}

%The study of human facial expressions and emotions never stops in our daily life while we communicate with others. Following the increased interest in automatic facial behavior analysis and understanding, the need of a semantic interpretation of the evolution of facial expressions and of human emotions has become of interest in recent years \cite{Fridlun2014}. In this paper, based on a work cooperated with the Serbian company 3Lateral, which has special expertise on building visual styles and designs in animation movies, we want to explore functional statistical instruments to identify the emotions while analyzing the expressions through recorded videos of human faces. The final aim of this research is to use this information to better and more realistically establish virtual digital characters, able to interact autonomously with real humans. 

%The data that we consider are multivariate longitudinal data, showing the evolution in time of different face muscles contraction. Functional Data Analysis (FDA) offers the possibility to analyze the entire expression evolution process over time and to gain detailed and in-depth insight into the analysis of emotion patterns. The basic idea in functional data analysis is that the measured data are noisy observations coming from a smooth function.  Ramsay and Silverman \cite{ramsay1997functional} describe the main features of FDA, that can be used to perform exploratory, confirmatory or predictive data analysis.  Ullah and Finch \cite{UllahShahid2013} published a systematic review on the applications of functional data analysis, where they included all areas where FDA was applied.

%Since the videos unavoidably have different beginning and ending points, the observed values are not comparable vertically among videos. Patterns of the expression functions common to each emotion are obscured due to the misalignment in the original data but can be clearer after curves are aligned\cite{marron2015functional}. It is essential to align the unregistered chronological timeline in the dataset into a common registered internal timeline that follows the same pronunciation speed, to control the influence of the speech itself, and then to study the influence of the emotions.

%From these $s_n$ curves, one can be interested in optimal representation of curves in a reduced dimensional function space (principal component analysis), or in classification, by determining an optimal partition of $\mathbf{Y}$ with respect to estimated coefficient functions. 


%\textbf{Overall/Pointwise ANOVA/MANOVA}

%\begin{itemize}
%   \item Overall: One conclusion for the whole evolution process: whether the additional emotion effect is zero or not.
%    \item Pointwise: Test the hypothesis $H_0$ at each time point, so that several discrete time zones are selected when the test is rejected. In these time zones, the emotion effect is treated to be significant.
%    \item ANOVA: Looking at single variate, in our case, one specific action unit per test. F test
%    \item MANOVA: Focus on multivariates, considering the mean and emotional effect as vectors of 17 action units together per test. Pillai test (Wilks test, LH test)
%\end{itemize}

%In our application, Functional ANOVA can be used to determine if there are time-related differences between emotion groups by using a functional F-test \cite{Dannenmaier2020}. Functional ANOVA yields the possibility to determine if a functional response can be described by scalar or functional variables.

%The structure of this paper goes as follows. In Section 2 we briefly describe the RAVDESS dataset from where the expression data of interest is extracted. Section 3 includes some methods of functional data analysis that we implemented in our application, and in Section 4 our results are presented.


%process:  After normalizing the curves representing the time series evolution in each set of observations, we then investigate if there exist patterns which could discriminate the different groups, using a FANOVA model.


%https://www.jwilber.me/permutationtest/



%Copy from the book of permutation test
The key underlying idea, on which the large majority of
testing solutions in multidimensional settings are based, is the nonparametric combination (NPC) of a set of dependent partial tests.

Observational studies have enjoyed increasing popularity in recent years for several reasons, including low costs and availability of large data sets, but they differ from experiments because there is no control of the assignment of treatments to subjects. In observational studies the experimenter’s main concern is usually to discover an association among variables of interest, possibly indicating one or more causal effects. The robustness of the nonparametric methodology against departures from normality and random sampling are much more relevant in observational studies than in controlled clinical trials.

Moreover, given that the NPC method is conditional on a set of sufficient statistics, it shows good general power behaviour, and the Fisher, Liptak or direct combining functions often have power functions which are quite close to the best parametric counterparts, when the latter are applicable, even for moderate
sample sizes. Thus NPC tests are relatively efficient and much less demanding in terms of underlying assumptions with respect to parametric competitors and to traditional distribution-free methods based on ranks, which are generally not conditional on sufficient statistics and so rarely present better unconditional power behaviour.

One major feature of the NPC with dependent tests,
provided that the permutation principle applies, is that we must pay attention to a set of partial tests, each appropriate to the related sub-hypotheses, because the underlying dependence relation structure (?) is nonparametrically and implicitly captured by the combining procedure. In particular, the researcher is not explicitly required to specify the dependence structure on response variables. This aspect is of great importance particularly for non-normal and categorical variables in which
dependence relations are generally too difficult to define, and, even when well defined, are hard to cope with. 


==> 2_data.tex <==

RAVDESS (Ryerson Audio-Visual Database of Emotional Speech and Song) \cite{livingstone2018ryerson} fits our needs for studying the human expression evolution and emotion identification, as it contains 24 professional actors (12 female, 12 male) to offer the performance with good quality and natural behavior under the emotions: calm, happy, sad, angry, fearful, disgusted and surprised. Also a neutral performance is available for each actor. The actors are vocalizing one lexically-matched statement in a neutral North American accent (“Kids are talking by the door”).

To avoid being lost in the difference of individual facial appearances, when analyzing the expressions and emotions, researchers mostly focus on the movements of individual facial muscles which are encoded by the Facial Action Coding System (FACS) \cite{ekman1997face}. FACS is a common standard to systematically categorize the physical expression of emotions, extracting the geometrical features of the faces and then producing temporal profiles of each facial movement. Such movements, corresponding to contraction of specific muscles of the face, are called \emph{action unit (AU)}.
%Using FACS human coders can manually code nearly any anatomically possible facial expression, deconstructing it into the specific action units and their temporal segments that produced the expression. Action units are a contraction or relaxation of one or more muscles. 
As action units are independent of any interpretation, they can be used for any higher-order decision-making process including recognition of basic emotions. Following the FACS rules, OpenFace \cite{amos2016openface}, an open-source software, is capable of recognizing and extracting facial action unit from facial images or videos. We applied OpenFace to extract the engagement degrees of action units for the videos in RAVDESS. The extracted action units include 17 functions for each video, taking values in $[0,5]$, sampled in about 110 time points (which is also the number of frames in each video). 

%As shown in Figure \ref{fig:EmosForOriginalCurves}, for different actors (in colors), different emotions (neutral as 1, angry as 4), the action units values change in different tendencies. Even for the performances of the same actor under same conditions, the repetition (solid and dash lines) slightly influences the values.




%\iffalse

%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{images/AUVSemoVSactorintensity2state1.pdf}
%\end{center}
%\caption{Five AUs values along time in the videos of all actors speaking statement "Kids are talking by the door" with strong intensity. AU01, 02, 04, 05, 06 represent respectively Inner Brow Raiser, Outer Brow Raiser, Brow Lowerer, Upper Lid Raiser, Cheek Raiser.}
%\label{fig:AUforall}
%\end{figure}

%\fi


==> 5_results.tex <==
%\subsection{Video Alignment}


%\url{https://hal.archives-ouvertes.fr/hal-00943745/document}
We will represent the action units evolution recorded on each video as a multivariate curves $\mathbf{Y}(t)= {[\mathbf{y}_{1}(t), \dots, \mathbf{y}_{D}(t)]^T, t \in [0, T]}$ ($D=17$ in our case). The observation of $\mathbf{Y}$ on our sample of videos provides the set ${\mathbf{Y_1},\dots, \mathbf{Y_n}}$ of multivariate curves, that we represent as multivariate functional data. 


As mentioned before, we first aligned the curves by separating the amplitude and phase variability. We choose to align the curves by AU25, which represents the lip movement, and then we adjusted the time frames of the other AUs according to this rescaling.

$(including neutral case when $g=0$)

%(see Figure \ref{fig:EmosForRegisteredCurves}).

%\begin{figure}[h]
%\centering
%\begin{subfigure}{.4\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{images/emo1original.png}  
%  \caption{The original curves).}
%  \label{fig:EmosForOriginalCurves}
%\end{subfigure}
%\begin{subfigure}{.4\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{images/emo1aligned.png}  
%  \caption{The registered curves.}
%  \label{fig:EmosForRegisteredCurves}
%\end{subfigure}

%\caption{Registration of AU25 for neutral and angry emotions. AU25 represents lips movement, which relates directly with the speech. The curves come from different videos.}
%\label{fig:EmosForCurves}
%\end{figure}

%Figure \ref{fig:EmosForCurves} illustrate the shapes of AU25 curves before and after the registration process. The x-axes "tstar" and "index" mean respectively the observed time before alignment and the common registered time after alignment, while the y-axis means the engagement degree of the AU25. After registration, the peaks of curves concentrate altogether on the same time points which are the pronunciation of some open-mouth syllables. Note that the first and last 30 time points are the breaks before starting and after ending of the speech respectively, so the variation does not influence the analysis of the speech part.

%By using the same standard rule of the match of the aligned timeline and original timelines for AU25, other AUs can add the standard aligned timeline, according to their original timelines and the matching relation as well. Thus we get the entire aligned dataset for the selected subset. By switching the labels, and repeating the operations above, we can get the aligned dataset as we want.


%After alignment, it's possible that one registered time point targets on several different AU values when the original timeline is compressed, so we do the linear interpolation and thus result in one "mean" approximation of these values as the single AU value at the registered time point. Then we are able to rebuild the dataset, using the commonly aligned frames as columns, while during this process the dataset contains many missing values, because each video has a different match to the registered timeline, so the interpolation is needed again. After removing the tail time points with useless missing values, we divide each AU value by the maximum value of the same AU in each video, to get a unified and normalized registered dataset.

We then applied the F-test described in the previous section to detect, for each emotion, which AUs have a mean behaviour significantly different from the neutral performance and in which time period during the videos.
In Figure \ref{fig:regression} we illustrate the results for emotion angry, as an example.

\begin{figure}[h]
\centering

\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au07ftest.png}  
  \caption{AU07.}
  \label{fig:07f}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au10ftest.png}  
  \caption{AU10.}
  \label{fig:10f}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au26ftest.png}  
  \caption{AU26.}
  \label{fig:26f}
\end{subfigure}

\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au07coeff.png}  
  \caption{AU07.}
  \label{fig:07c}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au10coeff.png}  
  \caption{AU10.}
  \label{fig:10c}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/au26coeff.png}  
  \caption{AU26.}
  \label{fig:26c}
\end{subfigure}

\caption{The functional coefficients  of action units 07 (Lid Tightener), 10 (Upper Lip Raiser) and 26 (Jaw Drop) under neutral and angry emotion and the corresponding F-test results}
\label{fig:regression}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{images/angryAUtimeline.png}  
    \caption{Which and where AU values are affected significantly by angry emotion }
    \label{fig:angry.timeline}
\end{figure}


The first row of Figure \ref{fig:regression} illustrates the estimated mean $\mu_0(t)$ (neutral emotion) and the angry emotion effects for three action units. The second row displays the observed F-statistics curves together with the pointwise and maximum 95\% quantile for the F-distribution in the dashed and horizontal dotted lines respectively. Thus  when the observed F-statistics is higher than the critical level lines, the emotion has a significant effect on the AU's pattern. We found in general three main situations of influence of one emotion on expression evolution: 1. locally strengthening (Figure \ref{fig:07c}: AU07 in frame range 45 to 55) 2. locally inhibiting (Figure \ref{fig:26c}: AU26 in frame range 70 to 90) 3. globally strengthening (Figure \ref{fig:10c}: AU10 in almost the whole time). Further, we pointed out the time zones of significant effects of the angry emotion on the action units in Figure \ref{fig:angry.timeline}, which is beneficial to understand and detect dynamically when and how the facial muscles contractions differ from the baseline.  


\begin{table}[htbp]
  \centering
  \small
  %\resizebox{0.6\textwidth}{!}{%
  \caption{Emotions with corresponding significant action units}
    \begin{tabular}{c|c}
    \hline
    \hline
    Emotions & Related Action Units\\
    \hline
    Calm  & $06, 07, 10, 12, 14, 23$\\
    Happy & $01, 06, 07, 10, 12, 14, 17, 23, 25, 26$ \\
    Sad   & $04, 06, 10, 14, 17, 20, 23, 25$ \\
    Angry & $04, 06, 07, 09, 10, 12, 14, 17, 23, 26$ \\
    Fearful & $04, 09, 10, 12, 14, 15, 17, 23, 25, 26$ \\
    Disgust & $04, 06, 07, 09, 10, 12, 14, 17, 23, 25, 26$ \\
    Surprised & $06, 09, 10, 12, 14, 15, 17, 23, 25, 26, 45$ \\
    \hline
    \hline
    \end{tabular}%
  \label{tab:emoau} %}
\end{table}

Table \ref{tab:emoau} summarizes for each emotion of interest the related action units that show significant changes from the neutral case  for our videos dataset. Similarly to the example of angry, we found that for happy and disgust emotions more action units have the globally strengthening effect on a large time range. Sad emotion sometimes affects the action units to be more constant than in neutral case. Emotion Fearful has more influence on upper half face (brows, eye lids and nose), while emotion calm is more related with the center of the face (Cheek Raiser, Lid Tightener and Lip Corner Puller). Surprised emotion is the only emotion where AU45 is significantly influenced. 

As a conclusion, our results can be joined in a multivariate setting and exploited to build a classifier able to automatically recognize the emotions. This task is left to subsequent works.




==> 6_simulation.tex <==

In this section, we want to explore, in consideration of knowing the ground-truth compositions of mean and kernel functions in groups, whether the proposed method of Functional ANOVA and Permutation tests works precisely and efficiently on different noise levels.
Thus, for the simulation settings, we generate 8 groups per variate to mimic the format of RAVDESS dataset. Figure \ref{fig:sim-org} gives an instance of the main trend functions (in blue) of sample curves in groups for one variate. Assume that each variate has a specific function indicating its original movement, i.e., one common mean function shared by all groups (in green). Each group has its own additional group-effect kernel function (in red), built on clear and independent time zones, so that we can easily conduct the important periods of the group's supplementary effect by default. The combination of the mean function and the additional kernel function indicates the main trend function of the corresponding group. Samples in that group are then generated by infusing the trend function with random white noise (Gaussian noise), and the sample size in one group per variate is set as 24. Multivariate case is obtained simply by repeating the process above several times. Here we show the results of 3-variate case. Meanwhile, other parameters fixed for this study include: permutation iterations to be 1000, quantile considered in permutation statistic's distribution to be 90\%.


%Figure \ref{fig:sim-org} gives an instance of the pairwise trend functions between one specific group (whose role is set as neutral group) and other groups, together with the default group-effect functions.


\begin{figure}
    \centering  
    \includegraphics[width=\linewidth]{image_final/EDA_ANOVA_simulation_original AU01_r.pdf}
    \caption{One exemplary variable of simulated data.}
    \label{fig:sim-org}
\end{figure} 


After the generation of simulated data, we build the FANOVA model introduced in the last section by transforming the time series data to functional data and estimating the parameter functions for common mean and additional group-effect kernels. Subsequently, we perform the corresponding statistical tests to detect the significant time zones in kernel functions. The detailed results of the estimated parameter functions and classic/permutation tests are shown in Figure \ref{fig:classic} and Figure \ref{fig:permutation_contrast} in the appendix respectively. We can observe that the classic test detects well the kernels when samples have small noise level, but turns to be worse quickly when noise level increases, while the permutation method is still able to detect the kernels on larger noise levels, although the estimated kernels are not as smooth as the original ones.

Further, with the adjustment of individual Gaussian noise levels, we define four measurements in order to explore further the pros and cons of test methods, such as kernel dissimilarities (the pointwise Euclidean distance between simulated and estimated kernels), significant time zone matching rate (how much significant time zones detected correctly), uni-classification correctness (classification only with one variate, the rate of correctly classified samples to the sample size) and multi-classification correctness (classification with all variates together). As illustrated in Figure \ref{fig:4measurements}, the kernel functions are detected better with permutation test than with classic F-test, especially when the noise reaches at a higher level. However, for classification correctness measurements, the differences are not as large as the kernels', althought when noise level being larger, the permutation method is more accurate than the classic one. From one side, this indicates the need to improve the classification process. Moreover, the reason to set critical value $\alpha = 0.1$ is restricted to the performance of classsic test results, since the classic test method with smaller critical value (e.g. $\alpha = 0.05$) often cannot distinguish the group-wise difference and detect no significant time zones when noise level is relatively large, so that we cannot continue the classification steps in that case. Therefore the other side is that considering the critical value ($\alpha = 0.1$) is relatively large for more complicated cases rather than this simplified simulation settings, the detection of kernels may give much worse classification result with classic F-test method in reality.



%3 test methods:
%\begin{itemize}
%    \item f test with full model and standard statistical table
%    \item f test with full model and permutation distribution
%    \item f test with bi-class model and permutation distribution
%\end{itemize}



%\ref{fig:sim-m1}: In the first tempts of simulation with univariate and multivariate constructed multiclass data, we have found that under the same condition with model's parameter setting and FANOVA processes, the samples in multivariate case reaches at better classification result than in univariate case.

\begin{figure}
    \centering 
        \begin{subfigure}{0.48\textwidth}
            \centering  
            \includegraphics[width=\linewidth]{image_final/N_KernelDissimilarities.pdf}
            \caption{Kernel Dissimilarities.}
            \label{fig:sim-m1}
        \end{subfigure}
        \begin{subfigure}{0.48\textwidth}
            \centering
            \includegraphics[width=\linewidth]{image_final/N_SignificantTimeZoneMatchingRate.pdf}
            \caption{Significant Time Zone Matching Rate.}
            \label{fig:sim-m2}
        \end{subfigure}
        \begin{subfigure}{0.48\textwidth}
            \centering  
            \includegraphics[width=\linewidth]{image_final/N_ClassificationCorrectness.pdf}
            \caption{Uni-Classification Correctness.}
            \label{fig:sim-m3}
        \end{subfigure}
        \begin{subfigure}{0.48\textwidth}
            \centering  
            \includegraphics[width=\linewidth]{image_final/N_MultiClassificationCorrectness.pdf}
            \caption{Multi-Classification Correctness.}
            \label{fig:sim-m4}
        \end{subfigure}
    \caption{Results of four measurements with different test methods.}
    \label{fig:4measurements}
\end{figure} 


%Next, instead of evaluating on variables, we explore the influences led by parameters from two aspects: the size of the sample (nobs) and the level of the coefficient of variation (CoV) in order to understand further the model's applicable scope.
%Adding the number of samples does not change the shape of kernels, but the smoothness of them.



    

 


==> 7_AUcasestudy.tex <==


\section{Data}

RAVDESS (Ryerson Audio-Visual Database of Emotional Speech and Song) \cite{livingstone2018ryerson} fits our needs for studying the human expression evolution and emotion identification, as it contains 24 professional actors (12 female, 12 male) to offer the performance with good quality and natural behavior under the emotions: calm, happy, sad, angry, fearful, disgusted and surprised. Also a neutral performance is available for each actor. The actors are vocalizing one lexically-matched statement in a neutral North American accent (“Kids are talking by the door”).

\section{AU Data Extraction}

To avoid being lost in the difference of individual facial appearances, when analyzing the expressions and emotions, researchers mostly focus on the movements of individual facial muscles which are encoded by the Facial Action Coding System (FACS) \cite{ekman1997face}. FACS is a common standard to systematically categorize the physical expression of emotions, extracting the geometrical features of the faces and then producing temporal profiles of each facial movement. Such movements, corresponding to contraction of specific muscles of the face, are called \emph{action unit (AU)}.
%Using FACS human coders can manually code nearly any anatomically possible facial expression, deconstructing it into the specific action units and their temporal segments that produced the expression. Action units are a contraction or relaxation of one or more muscles. 
As action units are independent of any interpretation, they can be used for any higher-order decision-making process including recognition of basic emotions. Following the FACS rules, OpenFace \cite{amos2016openface}, an open-source software, is capable of recognizing and extracting facial action unit from facial images or videos. We applied OpenFace to extract the engagement degrees of action units for the videos in RAVDESS. The extracted action units include 17 functions for each video, taking values in $[0,5]$, sampled in about 110 time points (which is also the number of frames in each video). 

%that follows the same pronunciation speed, to control the influence of the specific pronounced sentence and to detangle it from the influence of the emotions

\section{Heatmap}


\begin{itemize}
    \item Neutral: AU25,AU26 activated with small coefficient of variation; related with the sentence.
    \item Calm: AU7,AU12 slightly activated with small CV.
    \item Happy: AU12 highly activated with small CV, AU6,AU7,AU10,AU14 moderately activated with small CV.
    \item Sad: AU4,AU7 slightly activated with small CV
    \item Angry: AU7,AU10 moderately/slightly activated; AU4 slightly activated; AU25 is more activated than in neutral
    \item Fearful: AU4, AU7 slightly activated with small CV; other AUs tend to be activated in time zones where the CV is high, so not reliable; AU25, AU6 are less activated than in neutral, possibly because when you are fearful you tend to speak softly, moving less the mouth, so in this case we could consider also AU25, AU26 giving them a higher weight.
    \item Disgust: AU7,AU10 highly activated; AU4,AU6 moderately activated; AU14 slightly activated. all with small CV.
    \item Surprised: AU4,AU7 slightly activated with small CV; AU25,AU26 are less activated then neutral and could be considered.

\end{itemize}


\begin{figure}[h]
\centering

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/s1neutral.png}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1calm.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1happy.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1sad.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1angry.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1fearful.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1disgust.png}  
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/s1surprised.png}  
\end{subfigure}

\caption{Heatmaps of overall mean, overall coefficient of variation and self-defined normalization across emotions.}
\label{fig:heatmaps}
\end{figure}


\section{Results}

\begin{figure}[h]
\centering

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU04_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU04_r.pdf}  
  \caption{AU04}
  \label{fig:AU04}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU06_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU06_r.pdf}  
  \caption{AU06}
  \label{fig:AU06}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU07_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU07_r.pdf}  
  \caption{AU07}
  \label{fig:AU07}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU10_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU10_r.pdf}  
  \caption{AU10}
  \label{fig:AU10}
\end{subfigure}
\caption{Permutation test results and kernel functions (AU04,06,07,10).}
\label{fig:Permutationandkernel1}
\end{figure}

\begin{figure}[h]
\centering

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU12_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU12_r.pdf}  
  \caption{AU12}
  \label{fig:AU12}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU14_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU14_r.pdf}  
  \caption{AU14}
  \label{fig:AU14}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU25_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU25_r.pdf}  
  \caption{AU25}
  \label{fig:AU25}
\end{subfigure}
\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imagenew/ANOVA_perm_ AU26_r.pdf}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imagenew/ANOVA_regression_ AU26_r.pdf}  
  \caption{AU26}
  \label{fig:AU26}
\end{subfigure}

\caption{Permutation test results and kernel functions (AU12,14,25,26).}
\label{fig:Permutationandkernel2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imagenew/classification_results.png}
    \caption{Classification Results for AU dataset}
    \label{fig:classification.plots}
\end{figure}


==> 9_DetailsofResults.tex <==


\section{Details of Simulation Results}


\begin{figure}[h]
\centering

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_original AU01_r.pdf} 
    \caption{The original simulated data (Variate 1 for example)}
    \label{fig:simulated}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd0.05.pdf}
  \caption{sd 0.05.}
  \label{fig:sd0.05}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd0.5.pdf}  
  \caption{sd0.5.}
  \label{fig:sd0.5}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd1.pdf}  
  \caption{sd1.}
  \label{fig:sd1}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd2.pdf}  
  \caption{sd2.}
  \label{fig:sd2}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd3.pdf}  
  \caption{sd3.}
  \label{fig:sd3}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_folder_simulation6_classicftest/ANOVA_simulation_estimated AU01_r_sd4.pdf}  
  \caption{sd4.}
  \label{fig:sd4}
\end{subfigure}

\caption{The functional mean and additional effect coefficients for the comparison group and other groups through classic F-test with critical value $\alpha = 0.1$.}
\label{fig:classic}
\end{figure}


\begin{figure}[h]
\centering

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_original AU01_r.pdf} 
    \caption{The original simulated data (Variate 1 for example)}
    \label{fig:simulated}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd0.05.pdf}  
  \caption{sd 0.05.}
  \label{fig:sd0.05}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd0.5.pdf}  
  \caption{sd0.5.}
  \label{fig:sd0.5}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd1.pdf}  
  \caption{sd1.}
  \label{fig:sd1}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd2.pdf}  
  \caption{sd2.}
  \label{fig:sd2}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd3.pdf}  
  \caption{sd3.}
  \label{fig:sd3}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image_final/ANOVA_simulation_estimated AU01_r_sd4.pdf}  
  \caption{sd4.}
  \label{fig:sd4}
\end{subfigure}

\caption{The functional mean and additional effect coefficients for the comparison group and other groups through permutation test with contrast.}
\label{fig:permutation_contrast}
\end{figure}


\iffalse

\begin{figure}[h]
\centering
 \begin{subfigure}{0.32\textwidth}
            \centering  
            \includegraphics[width=\linewidth]{images/sd_nobs_kernelerror_nperm200.png}
            \subcaption{Kernel Dissimilarities.}
            \label{fig:sim-m1}
        \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/sd_nobs_timezoneerror_nperm200.png}
            \subcaption{Significant Time Zone Matching Rate.}
            \label{fig:sim-m2}
        \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
            \centering  
            \includegraphics[width=\linewidth]{images/sd_nobs_classification_nperm200.png}
            \subcaption{Uni-Classification Correctness.}
            \label{fig:sim-m3}
        \end{subfigure}
        
\caption{Results of 3 Measurements with different sample sizes and noise levels.}
\label{fig:nobs24_old}
\end{figure}

%For the case with coefficient of variation changing as noise, when the noisy level increases, the significant time zones of the kernel functions are detected more accurately and continuously (which indicates the decreasing effect of overfitting problem). However, the classification results go worse, probably because, even though the kernels' shapes are estimated well, the amplitude/absolute values of the functions become smaller, which would affect on the scanning process of the raw functions, so that the kernels show less power on the measuring part of classification. In a word, standard deviation influences not only on the selection of significant time zones, but also the amplitude of the function values. Adding the standard deviation helps to detect the significant time zones more accurately while it undermines the amplitude/power/influence of kernels, until the noisy level is so large that it disturbs the conveyed information to be meaningless.

\fi

%\section{Details of AU Data Results}







  
  

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The recommended style for references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}.} is depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI}.
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\end{thebibliography}

